Face Detection with Feature Pyramids and Landmarks

Accurate face detection and facial landmark localization are crucial to any face recognition system. We present a series of three single-stage RCNNs with different sized backbones (MobileNetV2-25, MobileNetV2-100, and ResNet101) and a six-layer feature pyramid trained exclusively on the WIDER FACE dataset. We compare the face detection and landmark accuracies using eight context module architectures, four proposed by previous research and four modified versions. We find no evidence that any of the proposed architectures significantly overperform and postulate that the random initialization of the additional layers is at least of equal importance. To show this we present a model that achieves near state-of-the-art performance on WIDER FACE and also provides high accuracy landmarks with a simple context module. We also present results using MobileNetV2 backbones, which achieve over 90% average precision on the WIDER FACE hard validation set while being able to run in real-time. By comparing to other authors, we show that our models exceed the state-of-the-art for similar-sized RCNNs and match the performance of much heavier networks.

==> backup_tables.tex <==
% \begin{tablehere}
% \captionsetup{justification=centering}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Head Module & AFW ($10^{-2}$) & AFLW ($10^{-2}$) \\
% \midrule
% SSH             & 1.14 $\pm$ 0.62 & 1.86 $\pm$ 2.80     \\
% SSH v2          & 1.55 $\pm$ 2.76 & 2.05 $\pm$ 2.42     \\
% Retina          & 1.12 $\pm$ 0.63 & 1.84 $\pm$ 2.68     \\
% Retina v2       & 1.09 $\pm$ 0.68 & 2.00 $\pm$ 3.15     \\
% RetinaSSH       & 1.11 $\pm$ 0.90 & 1.99 $\pm$ 3.09     \\
% RetinaSSH v2    & 1.12 $\pm$ 1.31 & 2.14 $\pm$ 3.33     \\
% Dense           & 1.15 $\pm$ 2.78 & 2.11 $\pm$ 3.16     \\
% Dense v2        & 1.27 $\pm$ 2.63 & 2.00 $\pm$ 2.92     \\
% \midrule
% Average         & 1.19 $\pm$ 1.80 & 2.00 $\pm$ 2.96    \\
% \bottomrule
% \end{tabular}
% \newline
% \caption{The mean absolute distance between the predicted landmark its ground truth, normalized by the bound box size, for each context module. The bottom row shows the average absolute error and the pooled standard deviation.}
% \label{tab:smalllmk}
% \end{tablehere}

% \begin{tablehere}
% \captionsetup{justification=centering}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Head Module & Hard AP \% ($\Delta$) & Overall AP  \\
% \midrule
% SSH             & 86.85 (+0.15) & 90.79 (-0.01)    \\
% SSH v2          & 86.76 (+0.06) & 90.86 (+0.05)    \\
% Retina          & 87.11 (+0.42) & 91.02 (+0.21)     \\
% Retina v2       & 87.27 (+0.57) & 91.03 (+0.22)   \\
% RetinaSSH       & 86.41 (-0.29) & 90.67 (-0.14)     \\
% RetinaSSH v2    & 86.67 (-0.03) & 90.83 (+0.02)    \\
% Dense           & 86.47 (-0.23) & 90.56 (-0.25)   \\
% Dense v2        & 86.05 (-0.65) & 90.70 (-0.11)     \\
% \midrule
% Average         & 86.70 $\pm$ 0.39 & 91.49 $\pm$ 0.16 \\
% \bottomrule
% \end{tabular}
% \newline
% \caption{The WIDER FACE validation average precision (AP) of the MobileNetV2 ($\alpha = 0.25$) backbone for each context module and their divergence from the mean ($\Delta$). The left column shows the performance on the `hard' set, and the right column shows the average performance across all three sets. The bottom row shows the mean AP and standard deviation for all the head modules.}
% \label{tab:smallwider}
% \end{tablehere}

% \begin{tablehere}
% \captionsetup{justification=centering}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Head Module & Hard AP \% ($\Delta$) & Overall AP ($\Delta$) \\
% \midrule
% SSH             &  89.04 (+0.11) & 92.76 (+0.14)    \\
% SSH v2          &  88.76 (-0.17) & 92.58 (-0.05)    \\
% Retina          &  88.87 (-0.06) & 92.59 (-0.04)     \\
% Retina v2       &  88.70 (-0.23) & 92.43 (-0.19)   \\
% RetinaSSH       &  89.19 (+0.26) & 92.69 (+0.06)     \\
% RetinaSSH v2    &  88.99 (+0.06) & 92.61 (-0.01)    \\
% Dense           &  88.93 (+0.00) & 92.57 (-0.05)   \\
% Dense v2        &  88.97 (+0.04) & 92.77 (+0.14)     \\
% \midrule
% Average         & 86.70 $\pm$ 0.16 & 91.49 $\pm$ 0.11 \\
% \bottomrule
% \end{tabular}
% \newline
% \caption{The WIDER FACE validation average precision (AP) of the MobileNetV2 ($\alpha = 1.0$) backbone for each context module and their divergence from the mean ($\Delta$). The left column shows the performance on the `hard' set, and the right column shows the average performance across all three sets. The bottom row shows the mean AP and standard deviation for all the head modules.}
% \label{tab:mediumwider}
% \end{tablehere}

% \begin{tablehere}
% \captionsetup{justification=centering}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Head Module & AFW ($10^{-2}$) & AFLW ($10^{-2}$) \\
% \midrule
% SSH             & 1.03 $\pm$ 056 & 1.60 $\pm$ 1.92     \\
% SSH v2          & 0.98 $\pm$ 098 & 1.51 $\pm$ 1.95    \\
% Retina          & 0.95 $\pm$ 059 & 1.63 $\pm$ 2.20     \\
% Retina v2       & 1.02 $\pm$ 057 & 1.61 $\pm$ 1.95     \\
% RetinaSSH       & 1.01 $\pm$ 052 & 1.42 $\pm$ 1.85     \\
% RetinaSSH v2    & 1.01 $\pm$ 099 & 1.54 $\pm$ 2.74     \\
% Dense           & 1.21 $\pm$ 066 & 1.58 $\pm$ 2.00     \\
% Dense v2        & 1.05 $\pm$ 139 & 1.48 $\pm$ 2.07     \\
% \midrule
% Average         & 1.03 $\pm$ 078 & 1.55 $\pm$ 2.10    \\
% \bottomrule
% \end{tabular}
% \newline
% \caption{The mean absolute distance between the predicted landmark its ground truth, normalized by the bound box size, for each context module. The bottom row shows the average absolute error and the pooled standard deviation.}
% \label{tab:mediumlmk}
% \end{tablehere}
